AskIt: Unified Programming Interface for Programming with Large Language Models

Large Language Models (LLMs) exhibit a unique phenomenon known as emergent abilities, demonstrating adeptness across numerous tasks, from text summarization to code generation. While these abilities open up novel avenues in software design and crafting, their incorporation presents substantial challenges. Developers face decisions regarding the use of LLMs for directly performing tasks within applications as well as for generating and executing code to accomplish these tasks. Moreover, effective prompt design becomes a critical concern, given the necessity of extracting data from natural language outputs. To address these complexities, this paper introduces AskIt, a domain-specific language (DSL) specifically designed for LLMs. AskIt simplifies LLM integration by providing a unified interface that not only allows for direct task execution using LLMs but also supports the entire cycle of code generation and execution. This dual capability is achieved through (1) type-guided output control, (2) template-based function definitions, and (3) prompt generation for both usage modes. Our evaluations underscore AskIt's effectiveness. Across 50 tasks, AskIt generated concise prompts, achieving a 16.14 % reduction in prompt length compared to benchmarks. Additionally, by enabling a seamless transition between using LLMs directly in applications and for generating code, AskIt achieved significant efficiency improvements, as observed in our GSM8K benchmark experiments. The implementations of AskIt in TypeScript and Python are available at https://github.com/katsumiok/ts-askit and https://github.com/katsumiok/pyaskit, respectively.

==> Makefile <==

SRCS := $(wildcard *.tex) $(wildcard fig/*) $(wildcard tab/*)
IMG_SRCS := $(wildcard fig/*.dot)
IMG_PDFS := $(patsubst %.dot,%.pdf,$(IMG_SRCS))

%.pdf: %.dot
	dot -Tpdf $< -o $@

# main.pdf: $(SRCS)
main.pdf: $(SRCS) $(IMG_PDFS)
	pdflatex main.tex
	bibtex main
	pdflatex main.tex
	pdflatex main.tex

clean:
	rm -rf `awk '/^\*/' .gitignore` main.pdf


==> tab/gsm8k.tex <==
\begin{tabular}{lrr}
\toprule
 & TypeScript & Python \\
Average Metrics &  &  \\
\midrule
Latency (s) & 13.36 & 22.97 \\
Execution Time (\si{\micro\second}) & 49.11 & 5.09 \\
Compilation Time (s) & 14.19 & 20.38 \\
Speedup Ratio & 276885.99 & 6969904.73 \\
\bottomrule
\end{tabular}


==> tab/humaneval_stats.tex <==
\begin{tabular}{lrrr}
\toprule
Metric & Original LOC & Processed LOC & LOC Ratio \\
\midrule
Average & 7.57 & 8.05 & 1.27 \\
Median & 7.00 & 8.00 & 1.00 \\
Minimum & 2.00 & 2.00 & 0.20 \\
Maximum & 30.00 & 35.00 & 6.00 \\
\bottomrule
\end{tabular}


==> tab/openai_evals.tex <==
\begin{tabular}{llrrr}
\toprule
Benchmark ID & Return Type & Original Length & Reduced Length & Percentage Reduction \\
\midrule
2d\_movement.dev.v0 & \texttt{object} & 506 & 387 & 23.52 \\
3d\_globe\_movement.dev.v0 & \texttt{string} & 633 & 549 & 13.27 \\
Unfamiliar-Chinese-Character.dev.v0 & \texttt{object} & 136 & 136 & 0.00 \\
aba\_mrpc\_true\_false.dev.v0 & \texttt{boolean} & 233 & 222 & 4.72 \\
abstract-causal-reasoning-symbolic.dev.v0 & \texttt{union} & 383 & 270 & 29.50 \\
abstract2title.test.v1 & \texttt{union} & 1531 & 1523 & 0.52 \\
actors-sequence.dev.match-v1 & \texttt{Array} & 403 & 304 & 24.57 \\
adultery\_state\_laws.dev.v0 & \texttt{Array} & 193 & 142 & 26.42 \\
afrikaans-lexicon.dev.v0 & \texttt{boolean} & 130 & 90 & 30.77 \\
aime\_evaluation.dev.v0 & \texttt{number} & 208 & 152 & 26.92 \\
algebra-word-problems.s1.simple-v0 & \texttt{number} & 211 & 136 & 35.55 \\
allergen-information.dev.v0 & \texttt{union} & 246 & 246 & 0.00 \\
alternate\_numeral\_systems.dev.v0 & \texttt{string} & 411 & 211 & 48.66 \\
ambiguous-sentences.dev.v0 & \texttt{string} & 134 & 134 & 0.00 \\
anagrams.test.v1 & \texttt{string} & 74 & 74 & 0.00 \\
arc.dev.v0 & \texttt{string} & 1070 & 1070 & 0.00 \\
arithmetic-expression-meta.dev.v0 & \texttt{string} & 601 & 441 & 26.62 \\
arithmetical\_puzzles.dev.v0 & \texttt{number} & 992 & 850 & 14.31 \\
ascii-digit-recognition.dev.v0 & \texttt{number} & 496 & 409 & 17.54 \\
ascii-wordart.dev.v0 & \texttt{string} & 815 & 807 & 0.98 \\
asl-classifiers.dev.v0 & \texttt{boolean} & 403 & 242 & 39.95 \\
atpl\_exams.dev.v0 & \texttt{union} & 693 & 625 & 9.81 \\
automata-and-complexity.dev.v0 & \texttt{boolean} & 283 & 128 & 54.77 \\
backgammon-illegal-move.dev.v0 & \texttt{boolean} & 743 & 621 & 16.42 \\
balance-chemical-equation.dev.v0 & \texttt{union} & 296 & 218 & 26.35 \\
base64-decode-simple.dev.v0 & \texttt{string} & 377 & 326 & 13.53 \\
beam.analysis.dev.v0 & \texttt{number} & 234 & 184 & 21.37 \\
belarusian-grammar.dev.v0 & \texttt{boolean} & 165 & 150 & 9.09 \\
belarusian-lexicon.dev.v0 & \texttt{boolean} & 108 & 93 & 13.89 \\
belarusian-numerals.dev.v0 & \texttt{number} & 246 & 179 & 27.24 \\
belarusian-orthography.dev.v0 & \texttt{string} & 218 & 218 & 0.00 \\
belarusian-proverbs.dev.v0 & \texttt{string} & 240 & 145 & 39.58 \\
belarusian-rhyme.dev.v0 & \texttt{union} & 180 & 159 & 11.67 \\
belarusian-russian-translation.dev.v0 & \texttt{string} & 347 & 347 & 0.00 \\
belarusian-syllable-count.dev.v0 & \texttt{number} & 169 & 127 & 24.85 \\
belarusian-synonyms.dev.v0 & \texttt{boolean} & 183 & 168 & 8.20 \\
benjaminmoore\_to\_hex.dev.v0 & \texttt{string} & 66 & 66 & 0.00 \\
best.dev.v0 & \texttt{string} & 35 & 35 & 0.00 \\
bigrams.dev.v0 & \texttt{number} & 300 & 300 & 0.00 \\
bitwise.dev.v0 & \texttt{string} & 502 & 502 & 0.00 \\
blackfoot-numerals-modern.dev.v0 & \texttt{number} & 707 & 305 & 56.86 \\
body-movement.dev.zero\_shot\_v0 & \texttt{union} & 510 & 465 & 8.82 \\
born-first.dev.v0 & \texttt{boolean} & 91 & 76 & 16.48 \\
brazilian-lexicon.dev.v0 & \texttt{boolean} & 138 & 98 & 28.99 \\
brazilian\_laws.test.v1 & \texttt{string} & 1068 & 1068 & 0.00 \\
building\_floorplan.test.v1 & \texttt{number} & 960 & 870 & 9.38 \\
bulgarian-lexicon.dev.v0 & \texttt{boolean} & 134 & 94 & 29.85 \\
canto\_wu\_pronunciation.dev.v0 & \texttt{string} & 301 & 301 & 0.00 \\
canto\_wu\_pronunciation\_fewshot.dev.v0 & \texttt{string} & 445 & 445 & 0.00 \\
\bottomrule
\end{tabular}


==> tab/reductions_table.tex <==
\begin{tabular}{llrrr}
\toprule
Benchmark ID & Return Type & Original Length & Reduced Length & Percentage Reduction \\
\midrule
2d\_movement.dev.v0 & \texttt{object} & 506 & 387 & 23.52 \\
3d\_globe\_movement.dev.v0 & \texttt{string} & 633 & 549 & 13.27 \\
Unfamiliar-Chinese-Character.dev.v0 & \texttt{object} & 136 & 136 & 0.00 \\
aba\_mrpc\_true\_false.dev.v0 & \texttt{boolean} & 233 & 222 & 4.72 \\
abstract-causal-reasoning-symbolic.dev.v0 & \texttt{union} & 383 & 270 & 29.50 \\
abstract2title.test.v1 & \texttt{union} & 1531 & 1523 & 0.52 \\
actors-sequence.dev.match-v1 & \texttt{Array} & 403 & 304 & 24.57 \\
adultery\_state\_laws.dev.v0 & \texttt{Array} & 193 & 142 & 26.42 \\
afrikaans-lexicon.dev.v0 & \texttt{boolean} & 130 & 90 & 30.77 \\
aime\_evaluation.dev.v0 & \texttt{number} & 208 & 152 & 26.92 \\
algebra-word-problems.s1.simple-v0 & \texttt{number} & 211 & 136 & 35.55 \\
allergen-information.dev.v0 & \texttt{union} & 246 & 246 & 0.00 \\
alternate\_numeral\_systems.dev.v0 & \texttt{string} & 411 & 211 & 48.66 \\
ambiguous-sentences.dev.v0 & \texttt{string} & 134 & 134 & 0.00 \\
anagrams.test.v1 & \texttt{string} & 74 & 74 & 0.00 \\
arc.dev.v0 & \texttt{string} & 1070 & 1070 & 0.00 \\
arithmetic-expression-meta.dev.v0 & \texttt{string} & 601 & 441 & 26.62 \\
arithmetical\_puzzles.dev.v0 & \texttt{number} & 992 & 850 & 14.31 \\
ascii-digit-recognition.dev.v0 & \texttt{number} & 496 & 409 & 17.54 \\
ascii-wordart.dev.v0 & \texttt{string} & 815 & 807 & 0.98 \\
asl-classifiers.dev.v0 & \texttt{boolean} & 403 & 242 & 39.95 \\
atpl\_exams.dev.v0 & \texttt{union} & 693 & 625 & 9.81 \\
automata-and-complexity.dev.v0 & \texttt{boolean} & 283 & 128 & 54.77 \\
backgammon-illegal-move.dev.v0 & \texttt{boolean} & 743 & 621 & 16.42 \\
balance-chemical-equation.dev.v0 & \texttt{union} & 296 & 218 & 26.35 \\
base64-decode-simple.dev.v0 & \texttt{string} & 377 & 326 & 13.53 \\
beam.analysis.dev.v0 & \texttt{number} & 234 & 184 & 21.37 \\
belarusian-grammar.dev.v0 & \texttt{boolean} & 165 & 150 & 9.09 \\
belarusian-lexicon.dev.v0 & \texttt{boolean} & 108 & 93 & 13.89 \\
belarusian-numerals.dev.v0 & \texttt{number} & 246 & 179 & 27.24 \\
belarusian-orthography.dev.v0 & \texttt{string} & 218 & 218 & 0.00 \\
belarusian-proverbs.dev.v0 & \texttt{string} & 240 & 145 & 39.58 \\
belarusian-rhyme.dev.v0 & \texttt{union} & 180 & 159 & 11.67 \\
belarusian-russian-translation.dev.v0 & \texttt{string} & 347 & 347 & 0.00 \\
belarusian-syllable-count.dev.v0 & \texttt{number} & 169 & 127 & 24.85 \\
belarusian-synonyms.dev.v0 & \texttt{boolean} & 183 & 168 & 8.20 \\
benjaminmoore\_to\_hex.dev.v0 & \texttt{string} & 66 & 66 & 0.00 \\
best.dev.v0 & \texttt{string} & 35 & 35 & 0.00 \\
bigrams.dev.v0 & \texttt{number} & 300 & 300 & 0.00 \\
bitwise.dev.v0 & \texttt{string} & 502 & 502 & 0.00 \\
blackfoot-numerals-modern.dev.v0 & \texttt{number} & 707 & 305 & 56.86 \\
body-movement.dev.zero\_shot\_v0 & \texttt{union} & 510 & 465 & 8.82 \\
born-first.dev.v0 & \texttt{boolean} & 91 & 76 & 16.48 \\
brazilian-lexicon.dev.v0 & \texttt{boolean} & 138 & 98 & 28.99 \\
brazilian\_laws.test.v1 & \texttt{string} & 1068 & 1068 & 0.00 \\
building\_floorplan.test.v1 & \texttt{number} & 960 & 870 & 9.38 \\
bulgarian-lexicon.dev.v0 & \texttt{boolean} & 134 & 94 & 29.85 \\
canto\_wu\_pronunciation.dev.v0 & \texttt{string} & 301 & 301 & 0.00 \\
canto\_wu\_pronunciation\_fewshot.dev.v0 & \texttt{string} & 445 & 445 & 0.00 \\
\bottomrule
\end{tabular}


==> tab/table.tex <==
1 &
    \begin{lstlisting}
    Reverse the string {{s}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    string
    \end{lstlisting}
    &
    \begin{lstlisting}
    { s: string }
    \end{lstlisting}
    & 5
    & 0
    & 4
    & 0
    \\ 
2 &
    \begin{lstlisting}
    Calculate the factorial of {{n}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number
    \end{lstlisting}
    &
    \begin{lstlisting}
    { n: number }
    \end{lstlisting}
    & 9
    & 0
    & 7
    & 0
    \\ 
3 &
    \begin{lstlisting}
    Concatenate the strings {{ss}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    string
    \end{lstlisting}
    &
    \begin{lstlisting}
    { ss: string[] }
    \end{lstlisting}
    & 5
    & 0
    & 4
    & 0
    \\ 
4 &
    \begin{lstlisting}
    Sort the numbers {{ns}} in ascending order.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number[]
    \end{lstlisting}
    &
    \begin{lstlisting}
    { ns: number[] }
    \end{lstlisting}
    & 5
    & 0
    & 5
    & 0
    \\ 
5 &
    \begin{lstlisting}
    Find the largest number in {{ns}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number
    \end{lstlisting}
    &
    \begin{lstlisting}
    { ns: number[] }
    \end{lstlisting}
    & 3
    & 0
    & 8
    & 0
    \\ 
6 &
    \begin{lstlisting}
    Check if {{n}} is a palindrome.
    \end{lstlisting}
    &
    \begin{lstlisting}
    boolean
    \end{lstlisting}
    &
    \begin{lstlisting}
    { n: number }
    \end{lstlisting}
    & 7
    & 0
    & 4
    & 0
    \\ 
7 &
    \begin{lstlisting}
    Calculate the sum of all numbers in {{ns}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number
    \end{lstlisting}
    &
    \begin{lstlisting}
    { ns: number[] }
    \end{lstlisting}
    & 5
    & 0
    & 4
    & 0
    \\ 
8 &
    \begin{lstlisting}
    Calculate the average of all numbers in {{ns}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number
    \end{lstlisting}
    &
    \begin{lstlisting}
    { ns: number[] }
    \end{lstlisting}
    & 8
    & 0
    & 7
    & 0
    \\ 
9 &
    \begin{lstlisting}
    Count the number of occurrences of {{x}} in {{xs}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number
    \end{lstlisting}
    &
    \begin{lstlisting}
    { xs: number[]; x: number }
    \end{lstlisting}
    & 6
    & 0
    & 8
    & 0
    \\ 
10 &
    \begin{lstlisting}
    Remove all instances of {{x}} from {{xs}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number[]
    \end{lstlisting}
    &
    \begin{lstlisting}
    { xs: number[]; x: number }
    \end{lstlisting}
    & 3
    & 0
    & 5
    & 0
    \\ 
11 &
    \begin{lstlisting}
    Return the unique elements in {{xs}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number[]
    \end{lstlisting}
    &
    \begin{lstlisting}
    { xs: number[] }
    \end{lstlisting}
    & 5
    & 0
    & 0
    & 0
    \\ 
12 &
    \begin{lstlisting}
    Find the factorial of {{n}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number
    \end{lstlisting}
    &
    \begin{lstlisting}
    { n: number }
    \end{lstlisting}
    & 9
    & 0
    & 7
    & 0
    \\ 
14 &
    \begin{lstlisting}
    Generate the Fibonacci sequence up to {{n}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number[]
    \end{lstlisting}
    &
    \begin{lstlisting}
    { n: number }
    \end{lstlisting}
    & 10
    & 0
    & 10
    & 7
    \\ 
21 &
    \begin{lstlisting}
    Convert the JSON object {{o}} into a string.
    \end{lstlisting}
    &
    \begin{lstlisting}
    string
    \end{lstlisting}
    &
    \begin{lstlisting}
    { o: any }
    \end{lstlisting}
    & 3
    & 0
    & 0
    & 0
    \\ 
24 &
    \begin{lstlisting}
    Find the difference between the dates {{d1}} and {{d2}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number
    \end{lstlisting}
    &
    \begin{lstlisting}
    { d1: Date; d2: Date }
    \end{lstlisting}
    & 6
    & 0
    & 0
    & 0
    

==> tab/table1.tex <==
1 &
    \begin{lstlisting}
    Reverse the string {{s}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    string
    \end{lstlisting}
    &
    \begin{lstlisting}
    { s: string }
    \end{lstlisting}
    & 5
    & 0
    & 4
    & 0
    \\ 
2 &
    \begin{lstlisting}
    Calculate the factorial of {{n}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number
    \end{lstlisting}
    &
    \begin{lstlisting}
    { n: number }
    \end{lstlisting}
    & 9
    & 0
    & 7
    & 0
    \\ 
3 &
    \begin{lstlisting}
    Concatenate the strings {{ss}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    string
    \end{lstlisting}
    &
    \begin{lstlisting}
    { ss: string[] }
    \end{lstlisting}
    & 5
    & 0
    & 4
    & 0
    \\ 
4 &
    \begin{lstlisting}
    Sort the numbers {{ns}} in ascending order.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number[]
    \end{lstlisting}
    &
    \begin{lstlisting}
    { ns: number[] }
    \end{lstlisting}
    & 5
    & 0
    & 5
    & 0
    \\ 
5 &
    \begin{lstlisting}
    Find the largest number in {{ns}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number
    \end{lstlisting}
    &
    \begin{lstlisting}
    { ns: number[] }
    \end{lstlisting}
    & 3
    & 0
    & 8
    & 0
    \\ 
6 &
    \begin{lstlisting}
    Check if {{n}} is a palindrome.
    \end{lstlisting}
    &
    \begin{lstlisting}
    boolean
    \end{lstlisting}
    &
    \begin{lstlisting}
    { n: number }
    \end{lstlisting}
    & 7
    & 0
    & 4
    & 0
    \\ 
7 &
    \begin{lstlisting}
    Calculate the sum of all numbers in {{ns}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number
    \end{lstlisting}
    &
    \begin{lstlisting}
    { ns: number[] }
    \end{lstlisting}
    & 5
    & 0
    & 4
    & 0
    \\ 
8 &
    \begin{lstlisting}
    Calculate the average of all numbers in {{ns}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number
    \end{lstlisting}
    &
    \begin{lstlisting}
    { ns: number[] }
    \end{lstlisting}
    & 8
    & 0
    & 7
    & 0
    \\ 
9 &
    \begin{lstlisting}
    Count the number of occurrences of {{x}} in {{xs}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number
    \end{lstlisting}
    &
    \begin{lstlisting}
    { xs: number[]; x: number }
    \end{lstlisting}
    & 6
    & 0
    & 8
    & 0
    \\ 
10 &
    \begin{lstlisting}
    Remove all instances of {{x}} from {{xs}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number[]
    \end{lstlisting}
    &
    \begin{lstlisting}
    { xs: number[]; x: number }
    \end{lstlisting}
    & 3
    & 0
    & 5
    & 0
    \\ 
11 &
    \begin{lstlisting}
    Return the unique elements in {{xs}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number[]
    \end{lstlisting}
    &
    \begin{lstlisting}
    { xs: number[] }
    \end{lstlisting}
    & 5
    & 0
    & 0
    & 0
    \\ 
12 &
    \begin{lstlisting}
    Find the factorial of {{n}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number
    \end{lstlisting}
    &
    \begin{lstlisting}
    { n: number }
    \end{lstlisting}
    & 9
    & 0
    & 7
    & 0
    \\ 
14 &
    \begin{lstlisting}
    Generate the Fibonacci sequence up to {{n}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number[]
    \end{lstlisting}
    &
    \begin{lstlisting}
    { n: number }
    \end{lstlisting}
    & 10
    & 0
    & 10
    & 7
    \\ 
21 &
    \begin{lstlisting}
    Convert the JSON object {{o}} into a string.
    \end{lstlisting}
    &
    \begin{lstlisting}
    string
    \end{lstlisting}
    &
    \begin{lstlisting}
    { o: any }
    \end{lstlisting}
    & 3
    & 0
    & 0
    & 0
    \\ 
24 &
    \begin{lstlisting}
    Find the difference between the dates {{d1}} and {{d2}}.
    \end{lstlisting}
    &
    \begin{lstlisting}
    number
    \end{lstlisting}
    &
    \begin{lstlisting}
    { d1: Date; d2: Date }
    \end{lstlisting}
    & 6
    & 0
    & 0
    & 0
    

==> tab/table2.tex <==
\begin{tabular}{llrrr}
\toprule
Benchmark ID & Return Type & Original Length & Reduced Length & Percentage Reduction \\
\midrule
2d\_movement.dev.v0 & \texttt{object} & 506 & 387 & 23.52 \\
3d\_globe\_movement.dev.v0 & \texttt{string} & 633 & 549 & 13.27 \\
Unfamiliar-Chinese-Character.dev.v0 & \texttt{object} & 136 & 136 & 0.00 \\
aba\_mrpc\_true\_false.dev.v0 & \texttt{boolean} & 233 & 222 & 4.72 \\
abstract-causal-reasoning-symbolic.dev.v0 & \texttt{union} & 383 & 270 & 29.50 \\
abstract2title.test.v1 & \texttt{union} & 1531 & 1523 & 0.52 \\
actors-sequence.dev.match-v1 & \texttt{Array} & 403 & 304 & 24.57 \\
adultery\_state\_laws.dev.v0 & \texttt{Array} & 193 & 142 & 26.42 \\
afrikaans-lexicon.dev.v0 & \texttt{boolean} & 130 & 90 & 30.77 \\
aime\_evaluation.dev.v0 & \texttt{number} & 208 & 152 & 26.92 \\
algebra-word-problems.s1.simple-v0 & \texttt{number} & 211 & 136 & 35.55 \\
allergen-information.dev.v0 & \texttt{union} & 246 & 246 & 0.00 \\
alternate\_numeral\_systems.dev.v0 & \texttt{string} & 411 & 211 & 48.66 \\
ambiguous-sentences.dev.v0 & \texttt{string} & 134 & 134 & 0.00 \\
anagrams.test.v1 & \texttt{string} & 74 & 74 & 0.00 \\
arc.dev.v0 & \texttt{string} & 1070 & 1070 & 0.00 \\
arithmetic-expression-meta.dev.v0 & \texttt{string} & 601 & 441 & 26.62 \\
arithmetical\_puzzles.dev.v0 & \texttt{number} & 992 & 850 & 14.31 \\
ascii-digit-recognition.dev.v0 & \texttt{number} & 496 & 409 & 17.54 \\
ascii-wordart.dev.v0 & \texttt{string} & 815 & 807 & 0.98 \\
asl-classifiers.dev.v0 & \texttt{boolean} & 403 & 242 & 39.95 \\
atpl\_exams.dev.v0 & \texttt{union} & 693 & 625 & 9.81 \\
automata-and-complexity.dev.v0 & \texttt{boolean} & 283 & 128 & 54.77 \\
backgammon-illegal-move.dev.v0 & \texttt{boolean} & 743 & 621 & 16.42 \\
balance-chemical-equation.dev.v0 & \texttt{union} & 296 & 218 & 26.35 \\
base64-decode-simple.dev.v0 & \texttt{string} & 377 & 326 & 13.53 \\
beam.analysis.dev.v0 & \texttt{number} & 234 & 184 & 21.37 \\
belarusian-grammar.dev.v0 & \texttt{boolean} & 165 & 150 & 9.09 \\
belarusian-lexicon.dev.v0 & \texttt{boolean} & 108 & 93 & 13.89 \\
belarusian-numerals.dev.v0 & \texttt{number} & 246 & 179 & 27.24 \\
belarusian-orthography.dev.v0 & \texttt{string} & 218 & 218 & 0.00 \\
belarusian-proverbs.dev.v0 & \texttt{string} & 240 & 145 & 39.58 \\
belarusian-rhyme.dev.v0 & \texttt{union} & 180 & 159 & 11.67 \\
belarusian-russian-translation.dev.v0 & \texttt{string} & 347 & 347 & 0.00 \\
belarusian-syllable-count.dev.v0 & \texttt{number} & 169 & 127 & 24.85 \\
belarusian-synonyms.dev.v0 & \texttt{boolean} & 183 & 168 & 8.20 \\
benjaminmoore\_to\_hex.dev.v0 & \texttt{string} & 66 & 66 & 0.00 \\
best.dev.v0 & \texttt{string} & 35 & 35 & 0.00 \\
bigrams.dev.v0 & \texttt{number} & 300 & 300 & 0.00 \\
bitwise.dev.v0 & \texttt{string} & 502 & 502 & 0.00 \\
blackfoot-numerals-modern.dev.v0 & \texttt{number} & 707 & 305 & 56.86 \\
body-movement.dev.zero\_shot\_v0 & \texttt{union} & 510 & 465 & 8.82 \\
born-first.dev.v0 & \texttt{boolean} & 91 & 76 & 16.48 \\
brazilian-lexicon.dev.v0 & \texttt{boolean} & 138 & 98 & 28.99 \\
brazilian\_laws.test.v1 & \texttt{string} & 1068 & 1068 & 0.00 \\
building\_floorplan.test.v1 & \texttt{number} & 960 & 870 & 9.38 \\
bulgarian-lexicon.dev.v0 & \texttt{boolean} & 134 & 94 & 29.85 \\
canto\_wu\_pronunciation.dev.v0 & \texttt{string} & 301 & 301 & 0.00 \\
canto\_wu\_pronunciation\_fewshot.dev.v0 & \texttt{string} & 445 & 445 & 0.00 \\
\bottomrule
\end{tabular}


==> tab/table3.tex <==
\begin{tabular}{lrr}
\toprule
 & TypeScript & Python \\
Average Metrics &  &  \\
\midrule
Latency (s) & 13.36 & 22.97 \\
Execution Time (\si{\micro\second}) & 49.11 & 5.09 \\
Compilation Time (s) & 14.19 & 20.38 \\
Speedup Ratio & 276885.99 & 6969904.73 \\
\bottomrule
\end{tabular}


==> tab/table_Python.tex <==
\begin{tabular}{lllllll}
\toprule
 & Retry Count & Latency [s] & Execution Time [us] & Compilation Time [s] & Recompilation Count & Speedup \\
\midrule
count & 1,134.00 & 1,134.00 & 1,134.00 & 1,134.00 & 1,134.00 & 1,134.00 \\
mean & 0.35 & 22.97 & 5.09 & 20.38 & 0.12 & 6,969,904.73 \\
%std & 0.95 & 19.49 & 27.87 & 32.25 & 0.69 & 6,663,536.00 \\
min & 0.00 & 4.08 & 0.50 & 3.90 & 0.00 & 15,069.51 \\
%25\% & 0.00 & 12.04 & 2.75 & 11.59 & 0.00 & 3,296,846.74 \\
%50\% & 0.00 & 16.57 & 3.50 & 15.62 & 0.00 & 5,043,720.84 \\
%75\% & 0.00 & 26.69 & 4.50 & 20.85 & 0.00 & 8,272,545.28 \\
max & 9.00 & 202.53 & 877.04 & 647.88 & 9.00 & 75,961,275.56 \\
\bottomrule
\end{tabular}


==> tab/table_TypeScript.tex <==
\begin{tabular}{lllllll}
\toprule
 & Retry Count & Latency [s] & Execution Time [us] & Compilation Time [s] & Recompilation Count & Speedup \\
\midrule
count & 1,114.00 & 1,114.00 & 1,114.00 & 1,114.00 & 1,114.00 & 1,114.00 \\
mean & 0.29 & 13.28 & 49.11 & 14.19 & 0.17 & 275,092.55 \\
%std & 0.85 & 10.27 & 16.35 & 12.70 & 0.83 & 205,078.71 \\
%min & 0.00 & 3.23 & 35.50 & 4.01 & 0.00 & 18,120.40 \\
%25\% & 0.00 & 7.57 & 43.76 & 9.12 & 0.00 & 162,877.58 \\
%50\% & 0.00 & 9.81 & 46.33 & 11.54 & 0.00 & 207,668.32 \\
%75\% & 0.00 & 15.43 & 50.20 & 14.89 & 0.00 & 314,665.95 \\
%max & 9.00 & 119.58 & 334.83 & 155.78 & 9.00 & 2,463,390.15 \\
\bottomrule
\end{tabular}

